Forward-backward stochastic differential equations with monotone functionals and mean field games with common noise

In this paper, we consider a system of forward-backward stochastic differential equations (FBSDEs) with monotone functionals. We show the existence and uniqueness of such a system by the method of continuation similarly to Peng and Wu (1999) for classical FBSDEs and obtain estimates under conditional probability. As applications, we prove the well-posedness result for a mean field FBSDE with conditional law and show the existence of a decoupling function. In addition, we show that mean field games with common noise are uniquely solvable under a linear controlled process with convex and weak-monotone cost functions and prove that the optimal control is in a feedback form depending only on the current state and conditional law.

==> texfiles/Mckean-Vlasov_system_test.tex <==
% !TEX root = main.tex

\begin{definition} Let $s \in [0,T], \xi \in \Ltwo_{\F_s}$ and $\{\G_t\}_{s \leq t \leq T}$ be a sub-filtration of $\{\F_t\}_{s \leq t \leq T}$. We define  \textit{FBSDE with data $(s,\xi,\{\G_t\}_{s \leq t \leq T})$} or simply \textit{FBSDE $(s,\xi,\{\G_t\}_{s \leq t \leq T})$} to be the following FBSDE
\begin{equation}\label{fbsde_gen}
	\begin{gathered}
dX_{t} = B(t, \theta_{t}, \mathcal{L}(X_{t}, Y_{t}|\tilde{\mathcal{F}}_{t}))dt + \Sigma(t, \theta_{t}, \mathcal{L}(X_{t}, Y_{t}|\tilde{\mathcal{F}}_{t}))dW_{t} + \epsilon(t, \theta_{t}, \mathcal{L}(X_{t}, Y_{t}|\tilde{\mathcal{F}}_{t}))d\tilde{W}_{t} \\
dY_{t} = F(t, \theta_{t}, \mathcal{L}(X_{t}, Y_{t}|\tilde{\mathcal{F}}_{t}))dt + Z_{t}dW_{t} + \tZ_{t}d\tilde{W}_{t}\\
X_{s} = \xi, \quad Y_{T} = G(X_{T}, \mathcal{L}(X_{T} | \tilde{\mathcal{F}}_{T}))
	\end{gathered}
\end{equation}
$\theta_{t} = (X_t,Y_t,Z_t,\tZ_t)_{s \leq t \leq T}$ is called a solution to FBSDE $(s,\xi,\{\G_t\}_{s \leq t \leq T})$ if they are $\F_t$-adapted and satisfy FBSDE \rref{fbsde_gen}.
\end{definition}



The assumptions are
\begin{assumpF}
$(f(t, X_{t}, Y_{t}, Z_{t},\tZ_{t}))_{0\leq t\leq T}$, for $f = b, \sigma, \epsilon$, and $(F(t, X_{t}, Y_{t}, Z_{t}, \tilde{Z}_{t},   \mathcal{L}(X_{t}, Y_{t}, Z_{t} , \tZ_{t}|\tilde{\mathcal{F}}_{t} ))_{0\leq t\leq T}$ are $\mathcal{F}_{t}$-progressively measurable for any  $\mathcal{F}_{t}$-progressively measurable.
\end{assumpF}

\begin{assumpF}
\begin{equation}
\int^{T}_{0}  |\phi(t, 0, 0, 0, 0, \delta_{0,0})|^{2}dt <\infty \quad\text{for }\phi=B, \Sigma,\epsilon, F
\end{equation}
\end{assumpF}



\begin{assumpF}
\begin{equation}
\begin{split}
&| \phi(t, \theta, m)  -  \phi(t, \theta', m')   |^{2} \leq K (|\Delta x|^{2}+ |b_{t}(\Delta y) + c_{t}(\Delta z) + d_{t}(\Delta \tz')|^{2} + W^{2}(m, m') )\quad \text{ for } \phi= B, \Sigma, \epsilon\\
&\Delta F_{t}^{2} \leq K ||\Delta\theta||^{2}+W^{2}(m, m')
\end{split}
\end{equation}
\end{assumpF}



\begin{assumpF}
$$ \mb{E}\l( \Ind_A\l[ \la \D F_t, \D X \ra + \la \D b_t, \D Y \ra +\tr \la \D \sigma_t, \D Z \ra +  \tr \la \D \epsilon_t, \D \tilde{Z} \ra \r] \r) 
	\leq  -\beta\mb{E}\l[ \Ind_{A}|b_t(\D Y)+c_t(\D Z) + d_{t}(\D \tilde{Z})|^2 \r], $$
for some $\beta > 0$ and
$$ \mb{E}[ \Ind_{B}\D G\D X ] \geq 0 $$
\end{assumpF}






Generally, to solve an FBSDE, we need to find what is called a \textit{decoupling field}, a possibly random function describing the relation of the backward process $Y_t$ as a function of the forward process $X_t$. When the coefficients are deterministic, this function is deterministic and is a solution to a quasilinear PDE. In that case, the FBSDE is said to be Markovian and we call the function a \textit{decoupling function}. Using this function, we can decouple an FBSDE and reduce the problem to solving a standard forward SDE. This method of solving FBSDE is called \textit{Four-steps scheme} and was first proposed by Ma et al. in \cite{ma1994solving}. See \cite{delarue2002existence} for more detail on a decoupling function of a classical FBSDE in a deterministic case and \cite{ma2011} for a decoupling field in a general case.

However, as $f,g$ are still deterministic functions of $m$, it is reasonable to expect a Markov property if we include an additional input, the current distribution of players, or in FBSDE context, the conditional law of $X_t$. Our main result for this section is the following theorem which shows the existence of a deterministic decoupling function for $\eps$-MFG thereby proving the Markov property of MFG with common noise.

\begin{thm}\label{ue_existence} There exist a deterministic function $U: [0,T] \times \R \times \Ptwo$ such that
 \begin{equation}\label{decouple_smp} 
 	Y_t = U(t,X_t,\Law(X_t|\tF_t))
\end{equation}
Moreover, $U$ satisfies the estimates
\begin{enumerate}
	\i $| U(t,x,m) - U(t,x',m')| \leq C_{K,T} \l( | x-x'| + \W_2(m,m') \r)$
	\i $\l( U(t,x,m)-U(t,x',m)\r)(x-x') \geq 0 $
\end{enumerate}
for all $t \in [0,T], x,x' \in \R, m,m' \in \Ptwo$ where $C_{K,T}$ depends only on $K,T$.
\end{thm}



Recall that $\tF^s_t$ is a $\sigma$-algebra generated by the common brownian motion starting at time $s$, i.e. $\tF^s_t = \sigma\l(\tW_r-\tW_s; s \leq r \leq t \r)$. For $\xi \in \Ltwo_{\F_s}$, we denote by $\theta^{s,\xi}_{t} =(X^{s,\xi}_t,Y^{s,\xi}_t,Z^{s,\xi}_t,{\tZ}^{s,\xi}_t)_{s \leq t \leq T}$ the unique solution to FBSDE $(s,\xi,\{\tF^s_t\}_{s \leq t \leq T})$, i.e. they satisfies 
\begin{equation}\label{fbsde_st}
	\begin{gathered}
dX^{s,\xi}_{t} = B(t, \theta^{s,\xi}_{t}, \mathcal{L}(X^{s,\xi}_{t}, Y^{s,\xi}_{t}|\tilde{\mathcal{F}}_{t}))dt + \Sigma(t, \theta^{s,\xi}_{t}, \mathcal{L}(X^{s,\xi}_{t}, Y^{s,\xi}_{t}|\tilde{\mathcal{F}}_{t}))dW_{t} + \epsilon(t, \theta^{s,\xi}_{t}, \mathcal{L}(X^{s,\xi}_{t}, Y^{s,\xi}_{t}|\tilde{\mathcal{F}}_{t}))d\tilde{W}_{t} \\
dY^{s,\xi}_{t} = F(t, \theta^{s,\xi}_{t}, \mathcal{L}(X^{s,\xi}_{t}, Y^{s,\xi}_{t}|\tilde{\mathcal{F}}_{t}))dt + Z^{s,\xi}_{t}dW_{t} + \tZ^{s,\xi}_{t}d\tilde{W}_{t}\\
X^{s,\xi}_{s} = \xi, \quad Y^{s,\xi}_{T} = G(X^{s,\xi}_{T}, \mathcal{L}(X^{s,\xi}_{T} | \tilde{\mathcal{F}}_{T}))
	\end{gathered}
\end{equation}
We define, for $0 \leq  s\leq t \leq T$, the following maps
\begin{equation}\label{theta}
\begin{aligned}
	\Theta^{s,t}: & \Ptwo \to \Mt{\F^s_t} \\
				&m	\to \Law(X^{s,\xi}_t| \tF_t^s) 
\end{aligned}
\end{equation}
and
\begin{equation}\label{function V}
\begin{aligned}
	V^{s,t}: & \Ptwo \to \mathscr{L}^{2}_{\mathscr{F}^{s}_{t}}(\mathscr{P}_{2}(\R^{2n})) \\
				&m	\to \mb{P}_{(X^{s, \xi}_t,Y^{s, \xi}_t)|\tF_t^s}
\end{aligned}
\end{equation}

where $\xi \in \Ltwo_{\F_s}$ with $\Law(\xi) = m$. We will sometimes use the following notation
\begin{equation}\label{msmt} 
	m^{s,m}_t \triangleq  \Theta^{s,t}(m)
\end{equation} 

{\color{red} Weak Uniqueness (not proved)}

\begin{prop}\label{weakU} Suppose that $\xi_1,\xi_2 \in \Ltwo_{\F_s}$ such that $\Law(\xi_1| \tF^r_s)=\Law(\xi_2| \tF^r_s) \in \Mt{\F_s}$, then $\mb{P}_{(X^{s, \xi_{1}}_t,Y^{s, \xi_{1}}_t)|\tF_t^r} = \mb{P}_{(X^{s, \xi_{2}}_t,Y^{s, \xi_{2}}_t)|\tF_t^r}$, and in particular $\Law(X^{s,\xi_1}_t| \tF^r_t) = \Law(X^{s,\xi_2}_t| \tF^r_t)$ for all $t \in [s,T]$ where $\tX^{s,\xi_1}_t,\tX^{s,\xi_2}_t$ are as defined above.
\end{prop} 

\begin{prop}\label{est_theta_prop}
For $0 \leq s \leq t \leq T$, $m,m' \in \Ptwo$, there exists a constant $C_{K,T}$ that  depends only on $K,T$ such that
\begin{equation}\label{est_theta} 
\mb{E}\l[ \W_2(\Theta^{s,t}(m),\Theta^{s,t}(m')) \r] \leq C_{K,T}\W_2(m,m')
\end{equation}
and
\begin{equation}\label{est_functionV} 
\mb{E}\l[ \W_2(V^{s,t}(m),V^{s,t}(m')) \r] \leq C_{K,T}\W_2(m,m')
\end{equation}

\end{prop}

\begin{proof} Let $\xi,\xi'$ be arbitrary elements of $\Ltwo_{\F_s}$ with law $m,m'$. Let $(X_t,Y_t,Z_t,\tZ_t)_{0 \leq t \leq T}$ and $(X'_t,Y'_t,Z'_t,\tZ'_t)_{0 \leq t \leq T}$ denote the solutions of FBSDE \rref{fbsde_mfg} with initial $X_s=\xi,X'_s=\xi'$, then by the estimate \rref{estimate_diff_mvfbsde}, it follows that 
$$ \mb{E}[\W^{2}_2(V^{s,t}(m),V^{s,t}(m'))] \leq \mb{E}[(X_t-X'_t)^2] + \mb{E}[(Y_t-Y'_t)^2] \leq C_{K,T}\mb{E}[(\xi-\xi')^2] $$
for a constant $C_{K,T}$ depends only on $K,T$. Since $\xi,\xi'$ are arbitrary, we conclude that
$$  \mb{E}[\W_2(V^{s,t}(m),V^{s,t}(m'))] \leq C\W_2(m,m') $$ 

The proof of equation \rref{est_theta} is almost identical.
\end{proof}

We first state and prove a lemma which will be used later
\begin{lemma}\label{representation_m_xi} Consider a Polish and atomless probability space $\Omega$. For two measures $m_{1}, m_{2}\in \in \Ptwo$ satisfying $\W_2(m_{1}, m_{2})< \epsilon$, and any random variable $\xi$ that has distribution $m_{1}$, $\exists \eta$ such that $\eta$ has distribution $m_{2}$ and  $(\mb{E}[ ||\xi - \eta||^{2}     ])^{\frac{1}{2}} < \epsilon$
\end{lemma}
\begin{proof}
By the definition of Wasserstein metric, there exists a small enough positive number $\epsilon'$ and two random variables $X$ and $Y$ has distributions $m_{1}$ and $m_{2}$ respectively and satisfy
\begin{equation}
(\mb{E}[ ||X - Y||^{2}     ])^{\frac{1}{2}} < \epsilon - \epsilon'
\end{equation}
Now by the lemma ({\color{red} in the MFG note}, there exists a bijective mapping $\tau$ from $\Omega$ to $\Omega$ that is measurable, measure-preserving and satisfying
\begin{equation}
\mb{E}[ ||X \circ \tau- \xi||_{\infty}] < \epsilon'
\end{equation}
which implies

\begin{equation}
(\mb{E}[ ||X \circ \tau - \xi||^{2}     ])^{\frac{1}{2}} <  \epsilon'
\end{equation}
Since $\tau$ is measure-preserving, $Y \circ \tau $ also has distribution $m_{2}$ and
\begin{equation}
\begin{split}
&(\mb{E}[ ||X \circ \tau - Y \circ \tau ||^{2}     ])^{\frac{1}{2}} = (\mb{E}[ ||X - Y||^{2}     ])^{\frac{1}{2}}  < \epsilon - \epsilon'\\
\Longrightarrow&(\mb{E}[ ||\xi- Y \circ \tau ||^{2}     ])^{\frac{1}{2}} < \epsilon
\end{split}
\end{equation}
So we can use $Y \circ \tau $ as our $\eta$



\end{proof}


\begin{thm}\label{markovian_m} For any $m \in \Ptwo$ and $0 \leq  s \leq t \leq u \leq T$
\begin{equation}\label{consistent}  
	\Theta^{t,u}(\Theta^{s,t}(m))=\Theta^{s,u}(m)
\end{equation}
where $\Theta$ is as defined in \rref{theta}.
\end{thm}

\input{texfiles/proof_markov_theta.tex}




With similar proof, we have
\begin{thm}\label{markovian_functionV} For any $m \in \Ptwo$ and $0 \leq  s \leq t \leq u \leq T$
\begin{equation}\label{consistent}  
	V^{t,u}(\Theta^{s,t}(m))=V^{s,u}(m)
\end{equation}
where $\Theta$ and $V$ are as defined in \rref{theta} and \rref{function V}.
\end{thm}

 
 
 
Next, we let $\xi \in \Ltwo_{\F_s}$ and define $(X^{s,\xi,m}_t,Y^{s,\xi,m}_t,Z^{s,\xi,m}_t,{\tZ}^{s,\xi,m}_t)_{s \leq t \leq T}$ to be the $\F_t$-adapted solution to the following FBSDE
\begin{equation}\label{mkfbsde_sub}
	\begin{gathered}
 dX^{s,\xi,m}_t = B(t, \theta^{s, \xi, m}_{t}, V^{s,t}(m)) dt + \Sigma(t, \theta^{s, \xi, m}_{t}, V^{s,t}(m)) dW_{t} + \eps(t, \theta^{s, \xi, m}_{t}, V^{s,t}(m))  \tdW_{t} \\
 dY^{s,\xi,m}_t  =F(t, \theta^{s, \xi, m}_{t}, V^{s,t}(m)) dt + Z^{s,\xi,m}_t dW_{t} + \tZ^{s,\xi,m}_t\tdW_{t} \\
 X^{s,\xi,m}_s = \xi, \quad Y^{s,\xi,m}_T = \d{x}g(X^{s,\xi,m}_T,m^{s,m}_T) 
	\end{gathered}
\end{equation}

\begin{remark} The FBSDE \rref{mkfbsde_sub} is a classical FBSDE with random coefficients and not a McKean-Vlasov FBSDE since the stochastic law $(m^{s,m}_t)_{0 \leq t \leq T}$ in the system is given exogenously.
\end{remark}

To ensure the existence and uniqueness of the FBSDE above using Theorem \ref{wellposed_ind}, we need to specify an additional condition
\begin{assumpF}
For any $m\in\mathscr{P}_{2}(\R^{2n})$, 
$$  \la\D F_t, \D x \ra + \la \D b_t, \D y \ra +\tr \la \D \sigma_t, \D z \ra +  \tr \la \D \epsilon_t, \D \tilde{z} \ra  
	\leq  -\beta\mb{E}\l[ \Ind_{A}|b_t(\D y)+c_t(\D z) + d_{t}(\D \tz) |^2 \r], $$
for some $\beta > 0$ and
$$ \mb{E}[ \Ind_{B}\D G\D x ] \geq 0 $$
Here $\D F_t = F(t, x, y, z, \tz, m) - F(t, x, y, z, \tz, m)$, and $\D b_{t}, \D \Sigma_{t}, \D \epsilon_{t}, \D G$ are similarly defined.
\end{assumpF}



Note that the initial $\xi$ here is arbitrary and does not necessarily have law $m$. When $\xi=x$ is a constant, \rref{mkfbsde_sub} corresponds to the FBSDE from an individual control problem over $[s,T]$ given $(m^{s,m}_t)_{s \leq t \leq T}$ with initial state $X_s=x$. In that case, $Y^{s,x,m}_s$ is deterministic since it is $\F_s^s$-measurable. This fact allows us to define the following map 
\begin{equation}\label{def_ue}
\begin{aligned}
	U: &[0,T] \times \R \times \Ptwo \to \R \\
				&(s,x,m)\mapsto Y^{s,x,m}_s
\end{aligned}
\end{equation}


To complete the proof of the Markov property of FBSDE \rref{smp_mfg}, we are left to show \rref{decouple_smp}. We first state a necessary estimate for $U$. 

\begin{lemma}\label{estimate_ue} Let $U:[0,T] \times \R \times \Ptwo \to \R$ be as defined above, then it satisfies

\begin{enumerate}
	\i $| U(t,x,m) - U(t,x',m')| \leq C_{K,T} \l( | x-x'| + \W_2(m,m') \r)$ \label{diffUe2}
	\i $\l( U(t,x,m)-U(t,x',m)\r)(x-x') \geq 0 $ \label{convexUe2}
\end{enumerate}
for all $t \in [0,T], x,x' \in \R, m,m' \in \Ptwo$, where $C_{K,T}$ depends only on $K,T$.
\end{lemma}

\begin{proof}
The first estimate directly follows from estimate \rref{estimate_diff_ind} and \rref{est_theta}. Next, Let $(X_t,Y_t,Z_t,\tZ_t)_{s \leq t \leq T}$ and $(X'_t,Y'_t,Z'_t,\tZ'_t)_{s \leq t \leq T}$ denote the solutions to the FBSDE corresponding to the definition of $U(s,x,m)$ and $U(s,x',m)$ respectively. Let $\D X_t = X_t - X'_t$ and define similarly $\D Y_t, \D \d{x}f, \D \d{x}g$. Applying \ito's lemma to $\D X_t \D Y_t$ and using convexity assumption \ref{convex}, particularly inequality \rref{mon10_ind}, gives
\begin{align*}
\mb{E}[\D Y_s\D X_s] =\mb{E}[\D G\D X_T] -\mb{E}\l[ \int_s^T \D F_{t} \D X_t + \D B_{t} \D Y_t + \tr\left( \D \Sigma_{t} \D Z_{t}\right) + \tr\left(\D \epsilon_{t} \D \tZ_{t} \right)           dt \r]  \geq 0
\end{align*}
By definition of $U$ and the fact that it is deterministic, we deduce that
$$ U(s,x,m)-U(s,x',m)(x-x') \geq 0 $$
\end{proof}

Now we are ready to state and prove the existence of a deterministic decoupling function thereby establishing the Markov result. Using Theorem \ref{markovian_m} above, we can show \rref{decouple_smp} using a similar argument as was done for a classical FBSDE (see Corollary 1.5 in \cite{delarue2002existence} for instance).


\begin{thm}\label{markovian_main}  Let $s \in [0,T], m \in \Ptwo, \xi \in \Ltwo_{\F_s}$, consider $(m^{s,m}_t)_{s \leq t \leq T}$ and $(X^{s,\xi,m}_t,Y^{s,\xi,m}_t,Z^{s,\xi,m}_t,{\tZ}^{s,\xi,m}_t)_{s \leq t \leq T}$ as defined above, then it follows that for all $t \in [s,T]$
\begin{equation}\label{decouple_smp_2}
Y^{s,\xi,m}_t = U(t, X^{s,\xi,m}_t, m^{s,m}_t)
\end{equation}
\end{thm}

\begin{remark} \rref{decouple_smp} in Theorem \ref{ue_existence} follows from \rref{decouple_smp_2} by setting $s=0$ and $\Law(\xi)=m$.
\end{remark}
\input{texfiles/proof_markov_ue.tex}




==> texfiles/abstract.tex <==
\begin{abstract}
In this paper, we consider a system of forward-backward stochastic differential equations (FBSDEs) with monotone functionals. We show the existence and 
uniqueness of such a system by the method of continuation similarly to Peng and Wu (1999) for classical FBSDEs and obtain estimates under conditional 
probability.  As applications, we prove the well-posedness result for a mean field FBSDE with conditional law and show the existence of a decoupling 
function. In addition, we show that mean field games with common noise are uniquely solvable under a linear controlled process with convex and weak-monotone 
cost functions and prove that the optimal control is in a feedback form depending only on the current state and conditional law.        
\end{abstract}
